Auctus: A Dataset Search Engine for Data Augmentation

The large volumes of structured data currently available, from Web tables to open-data portals and enterprise data, open up new opportunities for progress in answering many important scientific, societal, and business questions. However, finding relevant data is difficult. While search engines have addressed this problem for Web documents, there are many new challenges involved in supporting the discovery of structured data. We demonstrate how the Auctus dataset search engine addresses some of these challenges. We describe the system architecture and how users can explore datasets through a rich set of queries. We also present case studies which show how Auctus supports data augmentation to improve machine learning models as well as to enrich analytics.

==> sections/acknowledgment.tex <==
This work was partially supported by the DARPA D3M program and NSF award OAC-1640864. Any opinions, findings, and conclusions, or recommendations expressed in this material are those of the authors and do not necessarily reflect the views of NSF and DARPA.

==> sections/conclusions.tex <==
\section{Concluding Remarks}
\label{sec:conclusions}

To the best of our knowledge, \systemname is the first
\dataset search engine for data augmentation.
%
The system has been
successfully deployed and is being used by D3M project
members. % program.
%
%We are currently working on a number of improvements
%
\systemname is under active development and we are working on many
improvements, from new discovery plugins to more sophisticated join
and union algorithms.
%
We note that, while our original motivation to build \systemname was to improve ML model
performance, the system can also be useful in many data
exploration and integration scenarios. 

==> sections/futurework.tex <==
\section{Challenges and Future Work}
\label{sec:discussion}

To the best of our knowledge, \systemname is the first
\dataset search engine for data augmentation.
%
The system has been
successfully deployed and is being used by D3M project
members. % program.
%
%We are currently working on a number of improvements
%
\systemname is under active development and we are working on many
improvements, from new discovery plugins to more sophisticated join
and union algorithms.
%
We note that, while our original motivation to build \systemname was to improve ML model
performance, the system can also be useful in many data
exploration and integration scenarios. 
%We would like to explore these in future work.
%

% First, \datasets on the Web can change location and be continuously updated,
% so it is important to keep track of these changes and update the medadata
% accordingly.
%
%Second,
There are many open research challenges.
%for \dataset search engines for augmentation.
Notably, real data is messy and noise in data can negatively
impact the quality of search results, leading to both false
positives and negatives.  Thus, research on techniques that
address data noise is needed.
%either automatically clean data or support approximate joins and unions
%data cleaning tasks is essential to provide better guarantees for
%the quality of the integration.
%
There are also many open questions about how to rank \datasets. Examples are how to take the reputation of a \dataset repository 
into account,  how to diversify results, 
%ranking diversity can be implemented to return potentially
%different data in the query results,
or how to prioritize augmentations that are more likely to improve accuracy~\cite{shah@vldb2017}.

%Challenges related to ML (\eg finding \datasets that will potentially
%increase model performance) --
%cite \url{https://adalabucsd.github.io/papers/2016_Hamlet_SIGMOD.pdf}
%and \url{http://www.vldb.org/pvldb/vol11/p366-shah.pdf};
%say we could apply some of these techniques, although
%they only work for some algorithms --  better explain that.

==> sections/relatedwork.tex <==
\section{Related Work} \label{sec:relatedwork}

\paragraph{\Dataset Search}
Many \dataset search engines have become recently available~\cite{chapman@2019}.
Cafarella et al.~\cite{cafarella@vldb2008}
proposed a system to perform
keyword search over a corpus of HTML tables. 
Kaggle allows users to search for datasets through facets. It also allows data exploration using spreadsheet and column summaries. However, it does not support spatial queries, search for related datasets or perform augmentation tasks. Google Dataset Search provides a clean and easy to use interface to search datasets on the web.  Nevertheless, the keyword-based search has very limited capabilities e.g. it does not support spatial-temporal queries. Also, it does not provide any visual summary or metadata, so users must download the data and use other tools to explore it. It is problematic since it is a crucial task when users are trying to find a useful dataset. Others tools like Data.gov has the same issue. Even though, it supports spatial queries, it still does not
support temporal queries, data exploration or support for data augmentation tasks.
%In addition to Google \Dataset Search, Google also introduced Goods, a \dataset search system to manage data generated and used within the company~\cite{halevy@sigmod2016}.
%There is also a plethora of open data portals based on data donations~(\eg~\cite{chicagoopendata,nycopendata,ukopendata}) that provide search capabilities.
%The search methodology available in all of these engines and portals is largely keyword-based over the metadata published by the data sources, which, as described earlier, can be incomplete or inconsistent. The keyword-based search does not consider potential data augmentation tasks either.
%

\paragraph{Data Integration}
%
Data augmentation for structured data requires
finding tables for data integration (join and union),
a problem that has been commonly studied in the database community.
%
However, existing work is focused on either entity-centric
\datasets (\eg HTML tables)~\cite{bhagavatula@idea2013,cafarella@vldb2009,
dassarma@sigmod2012,lehmberg@web2014,yakout@sigmod2012,
zhang@sigmod2013}, \ie their techniques require the presence of named entities,
or primary key/foreign key
relationships~\cite{fernandez@icde2018}.
On the other hand, \datasets published on open data platforms
may not have any entities, and the augmentation may not follow
a primary key/foreign key relationship. %(see Figure~\ref{fig:example-intro}).
%
The aforementioned systems also require the presence of all of the data for
finding potential joins and unions,
which is unrealistically expensive in the context
of a search engine for \datasets over the Web.
%
Some systems are not suitable for
real-time queries~\cite{cafarella@vldb2009,dassarma@sigmod2012}, 
or assume that the relationship between the input \inputdata and
the repository has been precomputed~\cite{bhagavatula@idea2013,dassarma@sigmod2012}.
In our context, this assumption may not hold:
\inputdata is potentially an unknown \dataset to 
the search engine.
Nargesian et al.~\cite{nargesian@vldb2018} proposed a framework for finding top-$k$ \datasets that can be concatenated (union) with an input \dataset. They used different notions of ``unionability'' and indices to improve search performance. However, their approach is focused on textual attributes only.

% Nargesian et al.~\cite{nargesian@vldb2018} proposed a framework for finding top-$k$ \datasets that can be concatenated (union) with an external input \dataset (\ie not present in the framework's repository). They used different notions of ``unionability'' (\eg based on value intersection and embedding vectors), and various indices to improve search performance. However, their approach is focused on textual attributes only.


==> sections/removed.tex <==
\hide{
The goal is to, given an input \dataset \inputdata and an optional query
\query, efficiently and effectively discover and rank a set \outputdata
of \datasets from the Web that can be integrated (join or union) to \inputdata.
}
%
To address the limitations discussed above, our approach:
%(Section~\ref{sec:discussion} discusses other research questions):
\hide{
\jf{this list raises a red flag to me: we were criticized before because reviewers did not see novelty -- if we emphasize join/union we run the risk of this happening again. I think we should emphasize the visual exploration, enabling users to find relevant results. Join/union queries are just a means for that. We should also emphasize temporal and spatial search}
\scq{done}
}
%
\begin{myitemize}
\item \textbf{Discovers \datasets on the Web.}
\systemname does not rely on the availability of \texttt{schema.org} annotations. It can connect to APIs to capture \datasets
from different repositories. Its infrastructure is extensible and
allows multiple discovery plugins to be implemented.
%
\item \textbf{Supports data discovery and visual exploration to enrich analytics.}
\systemname supports a rich set of data discovery queries. Besides keywords, users can explore dataset collections based on space, time, and data relationships. \systemname  also offers \hide{an intuitive and user-friendly search results interface} a user-friendly interface for search results.
Filters and data exploration capabilities help users select the most suitable datasets for their problems.
%Different visualizations are displayed according to the type of data such as maps and data summary views, so users can understand and evaluate them in a faster manner. The contribution of filters and data exploration capabilities help users not only to discover useful data but also to select the more suitable dataset to be join/union to the input dataset if necessary.
% JF: we can say extraction or inference?
\item \textbf{Automatically infers metadata from \datasets.}
%
Instead of relying on published metadata, \systemname profiles \datasets as they are discovered in a scalable\hide{and consistent} way to power the search engine.
%
\item \textbf{Supports join and union search queries.}
%
To support data augmentation tasks, queries can be issued to find \datasets that can be either joined or concatenated with \inputdata.
%
To make these queries efficient, we create \textit{data summaries} for the
discovered \datasets, and use them to perform join and union queries.
%

\end{myitemize}


\jf{need to rewrite the next 2 paragraphs to better highlight what the general problem is; I am not sure whether having named paragraphs helps here}
\paragraph{Augmenting Data to Improve Predictive Models}
Consider \hide{for example} the problem of predicting the number of daily bicycle trips in New York City (NYC).
The initial training data contains the daily numbers of bicycle trip crossing the East River Bridges (used as a proxy for the city) with corresponding temperatures for April 2020. 
%
To build a model that generalizes 
well, it is crucial to acquire data for more months and, possibly,  attributes other than temperature to use as model features.  
%
%make data-driven predictions or decisions.
%The input data, in turn, is divided into two (often disjoint) sets:
%he training set is the set of data points that is used to fit the parameters of the estimator and to learn the model, while the test set is used to evaluate how well the model performs on unseen data.
%When the performance of machine learning pipelines is not satisfactory, data scientists often use strategies such as hyper-parameter tuning, feature engineering, and 
While there are over 2,400 datasets in the NYCOpenData repository~\cite{nycopendata}, how can we find specific datasets to  improve this model?
%In such pipelines, if the model performance is not satisfactory, there are a few strategies that data scientists often use to improve its overall performance. \eg hyperparameter tuning, ensemble learning, and data augmentation.
Answering this question is challenging, and highlights the importance of  mechanisms that \textit{detect relevant datasets for machine learning problems.} 

%Here, we focus on \textit{data augmentation}, which consists of
%increasing either the number of data points (\ie rows) of the input
%data or the number of features (\ie attributes) of the existing data points~\cite{}. \fcnote{Citation?}
%In the former case, the main idea is to feed the model with a larger, diversified training data set so that it can learn from both the existing and new data samples, and thus provide improved predictions,
%while in the latter, the goal is to add new relevant features to the existing samples that could lead to improved predictions of the dependent target variable.
%
\hide{
\jf{ideally we should demonstrate the importance of mixing and matching different constraints -- space, time; for example maybe 
there are too many datasets that are joinable, but when we limit the search to NYC and a time period, we have a more manageable set -- and here we should focus on articulating the challenges/desiderata}
}

\paragraph{Discovering Data to Enrich Analytics} 
%\hide{\jf{describe vito's problem}
%\scq{Done}} 
There are also concerns about \hide{the spatio-temporal nature of}  datasets that  occur in a variety of spatially and temporally disaggregate levels. In particular, finding relevant data that is compatible spatially and temporally in order to enrich data analytics is not trivial. For example, \hide{while  analyzing conflict forecasting problems,} researchers who use predictive modeling for conflict forecasting problems, either to guide policy-making decisions or to assess theories of conflict ~\cite{d2020conflict}, often have to identify new data sources in disparate spatio-temporal resolutions, merge those data, and evaluate the contribution of different features. 
%
Concretely, most conflicts materialize as spatio-temporal events, and if they occur in different resolutions and must be analyzed in tandem, joining their corresponding datasets may be challenging. 
%
This is just an example of how handling spatio-temporal datasets for  analytics can be challenging. 

\paragraph{Data Disco
